BLINDTRUST: Oblivious Remote Attestation for Secure Service Function Chains

With the rapidly evolving next-generation systems-of-systems, we face new security, resilience, and operational assurance challenges. In the face of the increasing attack landscape, it is necessary to cater to efficient mechanisms to verify software and device integrity to detect run-time modifications. Towards this direction, remote attestation is a promising defense mechanism that allows a third party, the verifier, to ensure a remote device's (the prover's) integrity. However, many of the existing families of attestation solutions have strong assumptions on the verifying entity's trustworthiness, thus not allowing for privacy preserving integrity correctness. Furthermore, they suffer from scalability and efficiency issues. This paper presents a lightweight dynamic configuration integrity verification that enables inter and intra-device attestation without disclosing any configuration information and can be applied on both resource-constrained edge devices and cloud services. Our goal is to enhance run-time software integrity and trustworthiness with a scalable solution eliminating the need for federated infrastructure trust.

==> 3_preliminaries.tex <==
\section{Definitions and Preliminaries}

\subsection{Remote Attestation}

Within the realms of malware detection and verifying the correctness of platforms, remote attestation (RA) emerged as a simple challenge-response protocol to enable a trusted verifier ($\verifier$) to ascertain the integrity of an untrusted remote platform, called the prover ($\prover$). The RA protocol now lays the foundation of ever sophisticated security services, such as provable software updates, control-flow attestation (CFA)~\cite{abera2016c}, and proof of remote software execution~\cite{nunes2020apex}. The general idea of the RA protocol is for $\verifier$ to send a challenge (\emph{nonce}) to $\prover$ and $\prover$ to respond with a \emph{nonce}-based authenticated integrity check over some resource (e.g., a memory region). $\verifier$ then determines whether the response is as expected (e.g., by comparing it to known reference values), and if so, $\verifier$ is confident that the $\prover$'s state is correct.

A more privacy-centered RA scheme is one where verifiers do not necessarily need any reference values.

To achieve RA in general, the attestation agent code should be \emph{immutable}, ... ~\cite{francillon2014minimalist}.

However, since we target containerized applications and their configurations, we can achieve many of these guarantees by virtually moving them outside the untrusted environment.


\subsection{Trusted Platform Modules}

Briefly mention difference between a TPM and a vTPM.

\subsubsection{Monotonic Counters}

Internally, each TPM has several PCRs that can be used for recording irreversible measurements through accumulation, e.g., extending PCR slot $i$ with measurement $m$, the TPM accumulates: $PCR_i = \hash(PCR_i \, \concat \, m)$. This is an indispensable property towards the creation of strong and transitive CoT. For instance, to enforce and regulate trustworthiness of the system boot sequence we can require that all components measure and verify their successors by the following recurrence construct: $I_0 = \true; I_{i+1} = I_i \land V_i(L_{i+1})$, where $i \leq n \land n \in \NN^*$, $I_i$ denotes the integrity of layer $i$ and $V_i$ is the corresponding verification function which compares the hash of its successor with a trusted reference value. For example, let us assume that we require the boot sequence: $\langle sinit,\allowbreak BL(m),\allowbreak OS(m),\allowbreak VM(m),\allowbreak APP(m) \rangle$, where $sinit$ is the value that the PCR is reset to. If we know that the sequence will yield PCR extensions with the values $v_1, \ldots, v_n$, and all components extend PCR $j$, then we will trust the chain \emph{if and only if (iff)} $PCR_j = \hash(\ldots(\hash(sinit\, \concat \, \hash(v_1)) \, \concat \, \hash(v_2))\ldots \, \concat \, \hash(v_n))$.

\subsubsection{Chain of Trust}

Transitive trust 


\subsubsection{Extended Authorization (EA)}
\label{subsubsec:extendedAuthorization}

``A good rule of thumb for attestation is that any machine authentication activity, when performed with a state-constrained key, provides attestation. A signing key with state constraint X will, when used, provide proof that at the time an object was signed, the PCR contents were compatible with X. An encryption key with state constraint Y will only decrypt the data if the PCR contents are compatible with Y''

Shifting from static (immutable) policies to flexible (mutable) policies.

\emph{wild card} policy, which is owned by a private key whose public key is associated with the wild card


\paragraph{Policy Assertions}

Immediate/deferred/hybrid

PolicyAuthorize vs PolicyAuthorizeNV. We opted for the former while preserving the revocability property of the latter. Instead of confining policies to NV indices, thus increasing the consumption of NV memory, we implicitly revoke policies by requesting and witnessing that the $\vf$ extends the NV index, which ensures that that policy cannot be fulfilled. However, if the $\orc$ is blocked from sending this request, the old policy will remain true. One solution to this would be to make the policy only valid within a certain time window. TOTP sync?

By binding a flexible authorization policy to NV indices, 
\begin{equation}
\begin{split}
\set{PolicyAuthorize} \land \{PolicyCommandCode(\\CC_{NV\_UndefineSpaceSpecial})\},
\end{split}
\end{equation}

\paragraph{Flexible policies}







==> 7_experiments.tex <==
\section{Performance Evaluation}

\subsection{Environmental Setup}
\label{subsec:environmentalSetup}

We implemented our protocols in C++ with IBM's TPM Software Stack (TSS) v1.6.0~\cite{ibmTsstpm} and OpenSSL v1.1.1i and compiled it using the GNU GCC compiler. We considered only elliptic curve (EC) keys and used SHA256 as $\mathcal{H}$. We tested the protocols on two platforms: (\emph{\textbf{P1}}) a computer running the Windows 10 OS, equipped with a 3.6 GHz AMD Ryzen 7 3700X CPU, and running IBM's SW TPM v1637~\cite{ibmTsstpm}, and (\emph{\textbf{P2}}) a Raspberry Pi 4 Model B Rev 1.4 with an 1.5Ghz ARM Cortex-A72 CPU running the Raspbian (buster) OS with an TPM 2.0 compliant OPTIGA HW TPM SLB9670.

% OS for benchmarking the protocols on an SW TPM. The code, together with OpenSSL 1.1.1i and IBM's TSS v1.6.0, is compiled using g++ v6.3.0 at optimization level 3 and runs against IBM's SW TPM (v1637) implementation of the TCG's TPM 2.0 specification~\cite{ibmTsstpm}. For the HW TPM benchmarking, we use a Raspberry Pi 4 Model B Rev 1.4 with a 1.5Ghz 64-bit quad-core ARM Cortex-A72 CPU and running the Raspbian GNU/Linux 10 (buster) OS. The code, together with IBM's TSS v1.6.0, is compiled using c++ v8.3.0 at optimization level 3 and runs against an attached OPTIGA HW TPM SLB 9670 TPM2.0. 


\subsection{Timing Tests}

Table~\ref{tab:appendixTimings} shows the mean (M) and standard deviations (SD) after running each protocol 50 times on each platform (Section~\ref{subsec:environmentalSetup}). The timings are produced using C++11's chrono library's system clock; each timing statistic includes time spent on the program code, TSS processing, the TPM's internal processing, and any Low Pin Count (LPC) bus delay (for \emph{\textbf{P2}}).

Note that although a security-centered HW-TPM is a bottleneck when it comes to efficiency, it provides security guarantees that a SW-TPM cannot. The most time-consuming protocols (i.e., AK creation, configuration updates, and NVPCR deletion) are those executed between $\orc$ and a $\vf$; thus, their efficiency has a negligible impact on the $\vf$ end. In ORA, which $\vf$s run among themselves, it takes a $\vf$ (with one active PCR, either normal or NV-based), $\approx$ 0.3s to perform the attestation using a HW-TPM and $\approx$ 12ms with a SW-TPM.

Appendix~\ref{appendix:timings}

% \begin{table}[htbp]
%     \caption{Timings (in ms) for each platform setup.}
%     \begin{center}
%         %\small
%         \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}} lrrrr}
%             \toprule
%             Protocol & M (\emph{\textbf{P1}}) & $\pm$SD & M (\emph{\textbf{P2}}) & $\pm$SD\\
%             \midrule
% \textbf{AK creation} & & & &\\
% \hspace{0.4cm}$\bm{\vf}$ & 15.22 & 1.21 & 543.89 & 5.99\\
% \hspace{0.4cm}$\bm{\orc}$ (verify) & 0.60 & 0.49 & 2.68 & 0.37\\
% \textbf{Measurement update} & & & &\\
% \hspace{0.4cm}$\bm{\vf}$ & 10.26 & 7.98 & 394.22 & 2.66\\
% \hspace{0.4cm}$\bm{\orc}$ (verify) & 0.48 & 0.50 & 2.46 & 0.05\\
% \textbf{ORA} & & & &\\
% \hspace{0.4cm}$\bm{\prover}$ & 12.32 & 21.9 & 327.21 & 2.18\\
% \hspace{0.4cm}$\bm{\verifier}$ (verify) & 0.52 & 0.50 & 2.42 & 0.05\\
% \textbf{Attaching NVPCR} & & & &\\
% \hspace{0.4cm}$\bm{\vf}$ & 11.40 & 0.63 & 117.9 & 1.28\\
% \hspace{0.4cm}$\bm{\orc}$ (verify) & 0.34 & 0.47 & 2.37 & 0.31\\
% \textbf{Detatching NVPCR} & & & &\\
% \hspace{0.4cm}$\bm{\vf}$ & 8.60 & 0.57 & 525.22 & 2.76\\
% % AK creation ($\vf\text{-side}$) & 15.22 & 1.21 & 543.89 & 5.99\\
% % Verify creation ($\orc\text{-side}$) & 0.60 & 0.49 & 2.68 & 0.37\\
% % Measurement update ($\vf\text{-side}$) & 10.26 & 7.98 & 394.22 & 2.66\\
% % Verify ($\orc\text{-side}$) & 0.48 & 0.50 & 2.46 & 0.05\\
% % ORA ($\prover\text{-side}$) & 12.32 & 21.9 & 327.21 & 2.18\\
% % Verify ($\verifier\text{-side}$) & 0.52 & 0.50 & 2.42 & 0.05\\
% % Attaching NVPCR ($\vf\text{-side}$) & 11.40 & 0.63 & 117.9 & 1.28\\
% % Verify ($\orc\text{-side}$) & 0.34 & 0.47 & 2.37 & 0.31\\
% % Detatching NVPCR ($\vf\text{-side}$) & 8.60 & 0.57 & 525.22 & 2.76\\
%             \bottomrule
%         \end{tabular*}
%         \label{tab:timings}
%     \end{center}
% \end{table}\normalsize








